Monocular 3D Object Detection via Geometric Reasoning on Keypoints

Monocular 3D object detection is well-known to be a challenging vision task due to the loss of depth information; attempts to recover depth using separate image-only approaches lead to unstable and noisy depth estimates, harming 3D detections. In this paper, we propose a novel keypoint-based approach for 3D object detection and localization from a single RGB image. We build our multi-branch model around 2D keypoint detection in images and complement it with a conceptually simple geometric reasoning method. Our network performs in an end-to-end manner, simultaneously and interdependently estimating 2D characteristics, such as 2D bounding boxes, keypoints, and orientation, along with full 3D pose in the scene. We fuse the outputs of distinct branches, applying a reprojection consistency loss during training. The experimental evaluation on the challenging KITTI dataset benchmark demonstrates that our network achieves state-of-the-art results among other monocular 3D detectors.

==> 03-framework-old.tex <==
\section{3D Object Detection Framework}
\label{sec:framework}










We propose an end-to-end trainable CNN-based framework that accepts a single RGB image as input and outputs 3D detections in the 3D scene. The network is split into two coherent sub-modules: firstly, 2D object and 2D keypoints detection and, secondly, 3D geometric reasoning, which includes localization derivation, dimensions and global orientation estimation. This section provides a detailed problem statement, followed by the description of the network sub-modules.


\subsection{Problem Definition}
\label{framework:problem-setup}

Given a single RGB image, our goal is to localize target objects in the 3D scene. Each target object is defined by its class and 3D bounding box, parameterized by 3D center coordinates $\textbf{C} = (c_x, c_y, c_z)$, assigned in a camera coordinate system, global orientation $\textbf{R} = (\theta, \cdot, \cdot)$, and dimensions $\textbf{D} = (w, h, l)$, standing for width, height and length, respectively (we don't correct for truncation or occlusion when defining object sizes). We parameterize global object orientation with the yaw angle $\theta$ only, which is a commonly adopted premise while dealing with objects on the road scenes~\cite{MousavianCVPR2017,qi2018frustum}. 

\subsection{Approach}
\label{framework:approach}

From the global perspective, the network comprises two sub-modules, each of which operates with the characteristics either 2D or 3D spaces. The gap between both spaces is filled by the instance depth retrieval, allowing to utilize monocular image-based 2D properties for the 3D localization. From the 2D perspective, each object of interest, cropped by the predicted bounding box, is provided with its keypoints 2D localization and their visibility state. The network also contains a branch with a local rotation angle prediction. The 3D sub-module focuses on direct dimension $\textbf{D}$ regression and CAD model assignment to the detected object out of the predefined set of the 3D meshes. Based on the pixel-meters height ratio between a selected pair of visible keypoints, extracted from both classified CAD model and height prediction, we retrieve the distance to an object, using camera parameters, known at each frame. This information is sufficient to obtain further the remaining 3D localization coordinates and global orientation.



\subsection{2D Detection}
\label{framework:2d-detection}

Our implementation follows and largely extends a two-stage network for object detection and instance segmentation - Mask R-CNN \cite{he2017mask}, which includes Feature Pyramid Network (FPN) \cite{lin2016feature}, Region Proposal Network (RPN) \cite{ren2015faster} and RoIAlign module \cite{he2017mask}. The RPN generates 2D anchor-boxes with a set of fixed aspect ratios and scales throughout the area of the provided feature maps, which are scored for the presence of the object of interest and adjusted. The spatial diversity of the proposed locations is processed by the RoIAlign block, converting each feature map, framed by the region of interest, into a fixed-size grid, preserving an  accurate spatial location through bilinear interpolation. Followed by fully connected layers, the network splits into two feature sharing branches for the bounding box regression and object classification. During training we utilize smooth L1 and cross-entropy loss for each task respectively, as defined in \cite{ren2015faster}.

\subsection{2D Keypoint Detection}
\label{framework:2d-keypoints}

We utilize the generality of the Mask R-CNN network in ability to extend to adjacent problem solutions. Instead of the human pose estimation via keypoints localization, considered in an original paper, we apply Mask R-CNN to car pose prediction. In addition, we drop the suggested parametrization via one-hot binary mask, in favour of a straightforward 2D pixel coordinates regression for each of $\textbf{K} = \{(x_i, y_i)_{i=1}^{14}\}$ keypoints (\eg, centers of 4 wheels, 4 corners of front and back windshields per each, centers of 2 headlights)\LA{provide a full enumeration if the keypoints are interpretable/meaningful}\IB{Provided all keypoints. The choice is explained in dataset description section}). We also supplement each keypoint coordinate with its visibility state, determined by the occlusion and truncation of an instance. Visibility is strictly a binary variable, setting no difference between occluded, self-occluded and truncated states\LA{is this our choice? what other things could have we chosen? why did we choose this particular option?} \IB{The binary visibility state is required both to propagate information during training for visible keypoints only and as an auxiliary supervision for local orientation branch quality enhancement}. During training, similar to 2D detection network head, we minimize the sum of regression and classification losses: smooth L1 loss for coordinates regression and log loss for visibility state classification, defined as follows:
\begin{equation}
\begin{aligned}
    &\mathcal{L}_{coord} = \sum\limits_{k=1}^K\mathbb{1}_k\cdot L_{1}^{smooth}\big(k^{gt}_{(x, y)},  k^{pred}_{(x, y)}\big)\\
    & \mathcal{L}_{vis} =  -\sum\limits_{k=1}^K \sum\limits_{j=1}^2 v^{gt}_{kj}\log v^{pred}_{kj}  \\
    &\mathcal{L}_{kp} = \mathcal{L}_{coord} + \mathcal{L}_{vis} \\
\end{aligned}
\end{equation}
where $\mathbb{1}_k$ is the visibility indicator of $k$-th keypoint, while $k^{gt}_{(x, y)}$ and $k^{pred}_{(x, y)}$ denote ground-truth and predicted 2D coordinates, normalized and defined in a fixed feature map grid coordinate system. Similarly, $v^{gt}_{kj}$ is the ground-truth visibility status, whilst $v^{pred}_{kj}$ is the estimated probability.

\subsection{3D Dimension and CAD Model Estimation}
\label{framework:3d-dim-cad-model}

The dimensions $\textbf{D}$ estimation sub-network operates in the same manner as the 2D bounding box localization. Instead of a regressing the absolute values, we predict the offsets to the mean values of each class of the CAD models, precomputed from the training dataset, along length, width and height. To train the network dimension branch, smooth L1 loss is adopted and defined as follows:
\begin{equation}
    \mathcal{L}_d = L_{1}^{smooth}\Big(\log\big(\textbf{D}^{gt}_{offset} - \textbf{D}^{pred}_{offset}\big)\Big)
\end{equation}
where $\textbf{D}^{gt}_{offset}$ and $\textbf{D}^{pred}_{offset}$ represent the ground truth and predicted offsets to the class mean values along each dimension respectively.

We force the network to share the same features for CAD model classification and dimension estimation in the common branch, due to the specificity of 3D CAD model registration to each ground truth car instance. 3D CAD model out of the predefined set of 5 templates is assigned, based on the width, length and height ratios. All the templates are presented on Fig. ~\ref{fig:pipeline}. During training we utilize multi-class log-loss.

\begin{figure}[t]
 \centering
 \includegraphics[width=0.5\textwidth, height=\textheight,keepaspectratio]{M3,3.png}
 \caption{Instance depth retrieval sub-module.}
  \label{fig:keypoints}
\end{figure}

\subsection{3D Location Estimation}
\label{framework:3d-location}

This sub-module extensively relies on the auxiliary network branches to estimate object's 3D center location $\textbf{C}$. The core component of the 3D location estimation is the instance depth retrieval, which is defined by the keypoints 2D localization branch, height prediction and CAD model classification. By instance depth here we mean the $Z$ coordinate of a vertical plane, relative to the origin of a camera coordinate system. From the pinhole camera model perspective, the distance to an instance is defined by the pixel-meters height ratio and the focal length of a camera. For a particular CAD model, given the height ratio $r^{k}_{cad}$ between the selected keypoints pair $k = \{(x_1, y_1),(x_2, y_2)\}$ in CAD model coordinate system, an estimated object height in meters $h_m$ from $\textbf{D}$, the keypoints pixel height $h^k_p$ and the distance to the object $Z$ are respectively defined as:
\begin{equation}
   h^k_p = |y_1 - y_2|,\hspace{4mm}Z = f \cdot\dfrac{r^{k}_{cad}\cdot h_m}{h^k_p}
\end{equation}
where $f$ is a focal length of camera, known for each frame. Fig.~\ref{fig:keypoints} provides a visualization for the depth retrieval sub-module. Depth coordinate $Z$ allows us to retrieve the remaining 3D location coordinates of one of the keypoints in a pair $k$, using the backprojection mapping:
\begin{equation}
   X = Z \cdot \dfrac{x_{\{1,2\}} - p_x}{f},\hspace{4mm} Y = Z \cdot \dfrac{y_{\{1,2\}} - p_y}{f}
\end{equation}
where $(p_x, p_y)$ are the camera principal point coordinates in pixels. To obtain finally the 3D bounding box center coordinates $\textbf{C}$, we utilize the rotation angle $\theta$, presented in the following subsection, as well as the distance between the keypoint and a car center. For a particular CAD model, given the weight, height and length ratio between the selected keypoint and car center $\textbf{r}_{cad} = (r^{w}_{k-c}, r^{h}_{k-c}, r^{l}_{k-c})$, estimated object dimensions $\textbf{D}$ and global orientation $\textbf{R}$, the car center $\textbf{C}$ is retrieved from the keypoint coordinate
\begin{equation}
    \textbf{C} = (X, Y, Z) \pm \textbf{R}\cdot  \textbf{D}*\textbf{r}_{cad}
\end{equation}
where $*$ stands for an element-wise product. Depending on the selected keypoint position (left or right car side, back or front, top or bottom), a sign is chosen for each dimension.

\begin{figure}[t]
 \centering
 \includegraphics[width=0.5\textwidth, height=\textheight,keepaspectratio]{annotation.png}
 \label{fig:annotation}
 \caption{An example of the keypoints annotation.}
\end{figure}

\subsection{Orientation Estimation}
\label{framework:orientation}

The straightforward $\textbf{R}$ estimation in a camera reference frame is not feasible, as the region proposal network propagates the context within the crops solely, cutting off the relation of the crop to the image plane. Inspired by Deep3DBox, we retrieve a global orientation as a combination of two angles, defined as follows:
\begin{equation}
\theta = \boldsymbol{\theta}_l + \boldsymbol{\theta}_{\text{ray}}
\end{equation}
where $\boldsymbol{\theta}_l$ is a local orientation of an object within the region of interest, whilst $\boldsymbol{\theta}_{\text{ray}}$ is a ray direction from camera to an object center. To accomplish the problem of $\boldsymbol{\theta}_l$ estimation, we adopt the MultiBin approach (Deep3DBox) with some minor modifications. In contrast to MultiBin, we avoid splitting the objective into an angle confidence and localization computation. Instead, we split the angle range from \ang{0} to \ang{360} degrees into 72 non-overlapping bins, obtaining the probability distribution over the discretized set as an output from the softmax layer. To train the local orientation network head, cross entropy is used as a loss function. $\boldsymbol{\theta}_{\text{ray}}$, in turn, directly follows from the 3D location coordinates.  

To deal with a single value not a probability distribution of a local orientation for the global yaw derivation, we utilize the weighted mean of the bins medians ($WM(\boldsymbol{\theta}_l)$), adopting the softmax output as the weights. Given 3D location coordinates $(X, Z)$ of one of the keypoints and the weighted mean local orientation $WM(\boldsymbol{\theta}_l)$, the global orientation is defined as follows:
\begin{equation}
\theta = WM(\boldsymbol{\theta}_l) +  \arctan\left(\dfrac{X}{Z}\right)
\end{equation}

\subsection{Multi-head Reprojection Consistency Loss}
\label{framework:reprojection-loss}

Except from shared convolutional blocks, each network branch is disconnected with its neighbours and is completely unaware of other predictions, though the geometric components are strictly tied to each other. To provide the consistency between the network branches, we introduce a loss function, which fuses all the predicted components. 3D coordinates in a CAD model coordinate system of the keypoints from the set $\textbf{K}$ are scaled, using $\textbf{D}$, rotated, using $\textbf{R}$, translated, using $\textbf{C}$, and backprojected into image plane via camera projection matrix to obtain 2D keypoints coordinates and compare with the ground truth values. A similar approach is applied to the 8 3D bounding box corners, straightforwardly obtained from $\textbf{C}$ and $\textbf{R}$, which should fit tightly into the ground truth 2D bounding box after backprojection. In both cases smooth L1 loss is used during training.

